Learning Transferable Cooperative Behavior in Multi-Agent Teams

While multi-agent interactions can be naturally modeled as a graph, the environment has traditionally been considered as a black box. We propose to create a shared agent-entity graph, where agents and environmental entities form vertices, and edges exist between the vertices which can communicate with each other. Agents learn to cooperate by exchanging messages along the edges of this graph. Our proposed multi-agent reinforcement learning framework is invariant to the number of agents or entities present in the system as well as permutation invariance, both of which are desirable properties for any multi-agent system representation. We present state-of-the-art results on coverage, formation and line control tasks for multi-agent teams in a fully decentralized framework and further show that the learned policies quickly transfer to scenarios with different team sizes along with strong zero-shot generalization performance. This is an important step towards developing multi-agent teams which can be realistically deployed in the real world without assuming complete prior knowledge or instantaneous communication at unbounded distances.

==> thesis_files/experiments.tex <==
% \begin{enumerate}
%     \item details like optimizers, policy network sizes etc.
%     \item generalization across agents
%     \item generalization across envt size
%     \item generalization after adding friction etc.
%     \item zero-shot generalization after removing (30,50,100\%) comms (in both with and w/o dropout masking during training
%     \item generalization across goals (threshold dist considered)?
%     \item specifically focus and comment on out-of-domain generalizations
%     \item zero-shot generalization and fine-tuned performance comparisons
%     \item comparisons with VAIN, CommNet, MADDPG, Q-Mix (?)
%     \item reward designs for simple spread
%     \item other environments apart from simple spread!
%     \item analysis of connectivity structure in masked 
%     \item hyperparam design choices?
%     \item comment bigger MPNN OR team spirit OR all the other things that didn't make a difference
% \end{enumerate}

\section{Environment Description}
\label{sec:task}

We present results on two standard swarm robotics tasks \cite{balch1998behavior,nagavalli2017automated}: coverage control and formation control. These are implemented inside the multi-agent particle environment \cite{lowe2017multi}, which is a 2-D world consisting of agents and landmarks in a continuous space with discrete time.

\subsubsection{Observation Space}
At each time step $t$, each agent observes only its own state $x_i^t \in \mathbb{R}^4$, comprising of 2D position and velocity. At the beginning of each episode, the agents also observe the positions of all entities (landmarks) in the environment, which are embedded as virtual nodes in the agent graph and used as described above.

\subsubsection{Action Space}
The agent has a discrete action space and chooses from 5 possible actions: (1) no-op, (2) $a_x = 1$, (3) $a_x = -1$, (4) $a_y = 1$, (5) $a_y = -1$ where $a_x,a_y$ represent accelerations in $x$ and $y$ dimensions, respectively, and $\textbf{a}^t = \begin{bmatrix} a_x \\ a_y \end{bmatrix} $ is used as input to the agent dynamics as shown below.

\subsubsection{Agent Dynamics}
Agents can move around in the 2-D space, and we provide a state space representation of the agent transition dynamics, where the state is denoted by $\textbf{y}$
\[
\textbf{y}_i^t = \begin{bmatrix} \textbf{p} \\ \textbf{p}^{'} \end{bmatrix}_i^t 
=  
\begin{bmatrix} \textbf{p}^{t-1} + \textbf{p}^{'} \Delta t \\ \gamma \textbf{p}^{'t-1} + \textbf{a}^t \Delta t \end{bmatrix}
\]
where $\textbf{p} \in \mathbb{R}^2$ is the 2-D position coordinates of the agent and $\textbf{p}^{'} \in \mathbb{R}^2$ is the 2-D velocity of the agent. $\gamma = 0.5$ is a damping coefficient used in double integrator robot dynamics models in the literature \cite{rao2001naive}. The agent chooses action $\textbf{a}^t$ at each time step $t$, and runs the simulation for $\Delta t = 0.1$s. We do not model collision dynamics.

\section{Task Description}
We now describe both the coverage and formation control tasks. 

\subsection{Coverage Control} 
\begin{figure}
    \centering
    \includegraphics[width=0.6\columnwidth]{figs/coverage_control.png}
    \caption{Coverage Control: 10 agents and 10 landmarks. Some landmarks have been covered, others have an agent on the way to cover them.}
    \label{fig:coveragecontrol}
\end{figure}
There are $M$ agents (blue) and $M$ landmarks (grey) in the environment, see Figure \ref{fig:coveragecontrol}. The objective is for the agents to deploy themselves in a manner to ensure that each landmark is covered, i.e. each landmark has at least one agent within a certain distance of it. The size of the environment is $4 \times 4$ unit square, and all the agent and landmark positions are randomly initialized at the beginning of each episode, so the learned policy does not depend on any particular configuration of the landmarks.
Note that we \textbf{do not assign particular landmarks to each agent}, as is the standard practice in the swarm robotics literature, but instead let the agents communicate with each other and develop a consensus about which agent will cover which landmark.

\subsubsection{Reward Function} 
At each time step $t$, we consider an agent-landmark bipartite graph, where the agents form one set of nodes $A$ and the landmarks for the other set of nodes $L$. There are weighted edges from every node in $A \rightarrow L$, with edge weights being specified by the $L_2$ distance. We then find the minimum weight matching, which is a set of edges without common vertices such that the combined weight of the edges is minimized.
Intuitively, this finds the agent closest to each landmark and considers the distance between this pair, while ensuring that the same agent does not count as being the closest agent to two different landmarks (i.e., we do not want the same agent to be able to cover two different landmarks at the same time).
We use the Hungarian algorithm \cite{kuhn1955hungarian} for linear sum assignment to find this minimum weight matching.
Finally, we use the negative of the clipped mean distance of a landmark to its closest agent (as specified by the linear assignment) as a shared reward function for the team.
This incentivizes the team to cooperatively cover all landmarks.

\subsubsection{Goal Specification}
The task is episodic, and can terminate for one of the following two reasons:
\begin{enumerate}
    \item Each landmark has at least one agent within a distance of $0.1$ units from it, where the overall size of the environment is $4 \times 4$ unit square. This is a success case.
    \item $50$ time steps have lapsed since the beginning of the episode without the agents having completed the task. This is a failure case.
\end{enumerate}

\subsection{Formation Control}
\begin{figure}[!b]
    \centering
    \includegraphics[width=0.6\columnwidth]{figs/formation_control.png}
    \caption{Formation Control: 10 agents coalescing to form a 10-sided regular polygon around the landmark.}
    \label{fig:formationcontrol}
\end{figure}
There are $M$ agents (blue) and $1$ landmark (grey) in the environment, see Figure \ref{fig:formationcontrol}. The objective is for the agents to deploy themselves into a $M$-sided regular polygonal formation, with the landmark at its centre. The size of the environment is $2 \times 2$ unit square, and all the agent and landmark positions are randomly initialized at the beginning of each episode.
Again, note that we do not specify any particular orientation to the polygon, or assign agents to specific points along that polygon - but instead let the agents communicate with each other to spread out uniformly.

\subsubsection{Reward Function}

The reward provided by the environment to the agents at each timestep is a sum of two terms: a radial separation reward, and an angular separation reward.
\begin{enumerate}
    \item \textbf{Radial Separation: }We specify a desired distance ($0.5$ units) that all agents should be from the landmark, and provide a clipped negative of the absolute value of the deviation from that distance as a reward to each agent. This term ensures that all agents are at the correct distance from the landmark, however it does nothing to spread them out uniformly.
    
    \item \textbf{Angular Separation: }Agents should be spread out at an angle of $\frac{2\pi}{N}$ to create a regular polygon ($N$ is the number of agents). We penalize the agents for deviating from this angle, ensuring that they spread out at the appropriate angle. We scale this term by $\frac{1}{\pi}$ so that both radial and angular separation terms have similar magnitude.
\end{enumerate}

\subsubsection{Goal Specification}

The task is episodic, and can terminate for one of the following two reasons:
\begin{enumerate}
    \item Each agent is within $\pm 0.05$ units of the target distance from the landmark, \textbf{AND} within $\pm 0.1 $ radians of the target angular separation. This is a success case.
    \item $50$ time steps have lapsed since the beginning of the episode without the agents having completed the task. This is a failure case.
\end{enumerate}
\section{Experimental Specifications}

\subsubsection{Network Architecture}
\begin{enumerate}
    \item Embedding dimension $H = 128$
    \item Agent state encoder, $q$: Single fully-connected layer (FC): $\mathbb{R}^4 \rightarrow \mathbb{R}^{128}$, followed by a rectified linear unit (ReLU) non-linearity
    \item Entity state encoder, $r$: Single FC layer + ReLU, $\mathbb{R}^2 \rightarrow \mathbb{R}^{128}$ 
    \item Environment encoder $D_K,D_V,D_Q = 128$
    \item Inter-agent communication $D_K,D_V,D_Q = 128$ for multi-head attention based communication with $C = 3$ hops.
    \item Agent state update function, $g$: Single fully-connected layer (FC) layer $\mathbb{R}^{256} \rightarrow \mathbb{R}^{128}$
    \item Value output head: FC layer + ReLU + FC layer, overall $\mathbb{R}^{128} \rightarrow \mathbb{R}^{1}$
    \item Policy output head: FC layer + ReLU + FC layer, overall $\mathbb{R}^{128} \rightarrow \mathbb{R}^{5}$
\end{enumerate}
All parameters are initialized using orthogonal initialization \cite{saxe2013exact}.

\subsubsection{Hyperparameters}
\begin{enumerate}
    \item For dropout communication, we drop 50\% edges which are randomly resampled every $10$ timesteps.
    \item We restrict communication to a radius of $R = 2$ units in the coverage control task, where arena size is $4 \times 4$, and to $R = 1$ unit in the formation control task, where arena size is $2 \times 2$.
    \item During training, agents collect experience from 32 environments in parallel, all initialized with different seeds 
    \item Each evaluation is in a newly initialized environment with different random seeds, following best practices for evaluation of reinforcement learning \cite{machado2018revisiting}.
    \item We use the Adam optimizer \cite{kingma2014adam} with learning rate $1e-4$.
    \item Future rewards are discounted with $\gamma = 0.99$
    \item The GAE parameter from Equation \ref{eq:gae} $\lambda = 0.95$
    \item Entropy coefficient $c_2$ from Equation \ref{eq:ppo} is 0.01
    \item Value loss coefficient $c_1$ from Equation \ref{eq:ppo} is 0.5
    \item Gradients were clipped to keep $L_2$ norms below 0.5
    \item Each batch of experience was used for $4$ PPO updates
    \item PPO clipping parameter $\epsilon$ from Equation \ref{eq:lclip} is 0.2
\end{enumerate}
The entropy coefficient and value loss coefficient values were obtained after minimal hyperparameter tuning on coverage control, while the other values were chosen based on previous work and publicly available implementations of RL algorithms. Note that we did not need to tweak any parameters for formation control.
\cite{pytorchrl}.

% \subsubsection{Curriculum Training}
% The underlying graph network representation we use to model the multi-agent interactions allows us to transfer learned policies to scenarios with different number of team mates. We exploit this to do curriculum learning, where a policy is trained from scratch for $M=3$ agents, then transferred (and fine-tuned) to $M=5$ agents, and so on.

\section{Results}
\label{sec:results}
We evaluate various learning methods on the following metrics:
\begin{enumerate}
    \item \textbf{Success Rate} ($\%$): In what percentage of episodes does the team achieve its objective? (Higher is better)
    \item \textbf{Time}: How many time steps does the team require to achieve its objective? (Lower is better)
    \item \textbf{Average Distance}: (for coverage control only) what is the average distance of a landmark to its closest agent?
\end{enumerate}
For evaluation, we pause each training run after 50 update steps and evaluate on 30 episodes in a newly seeded environment, with each agent performing greedy decentralized action selection. 

We present results of our graph network based learning framework on both tasks, with $N = \{3,\cdots,10\}$ agents, using the following abbreviations while reporting results with all 3 inter-agent communication functions discussed in Section \ref{sec:comms}: \texttt{MHA}: Multi-Head Attention, \texttt{EXP}: Exponential Kernel Attention \cite{hoshen2017vain}, \texttt{UNIFORM}: Uniform Attention \cite{sukhbaatar2016learning}. We also present results in 2 communication settings: (1) Unrestricted Communication (\texttt{UC}), where all agents can communicate with each other, and (2) Restricted Communication (\texttt{RC}), where agents can only communicate with other agents that are within their radius of communication ($R = 1$ unit distance).

\subsection{Comparisons with previous work}
\label{sec:comparisons}
While we could not find previous work on multi-agent reinforcement learning in coverage or formation control and hence do not have previously published results to compare with, we use publicly available implementations\footnote{\url{https://github.com/oxwhirl/pymarl}} to compare with Q-Mix \cite{rashid2018qmix}, VDN \cite{sunehag2017value}, IQL \cite{tampuu2017multiagent} and MADDPG \cite{lowe2017multi}. These methods rely on access to global state during training (and local state during execution), instead of inter-agent communication, for emergence of cooperation. Hence, at first, we restricted each agent to observe other agents only within a certain radius (while the global state with all agents and landmarks was available during training). However, none of the methods learn to complete the task ($0\%$ success), hence we relaxed the observability to be global for all agents - after which Q-Mix got to a $20\%$ success rate, with the other methods still unable to learn to cooperate successfully, see Table \ref{tab:prevwork}. By contrast, our methods easily outperforms previously proposed methods even with partial observability and restricted communication. We emphasize that the invariance of our method to the number of agents allows us to use curriculum learning and transfer learned policies from 3 to 6 agents, while the previous works use architectures that do not allow such transfer. Hence, in the presented results, with $M=6$ agents, our method has been bootstrapped from the $M=3$ case, while the previous works have been trained from scratch. However, considering the poor performance of those methods in the $M=3$ case, we do not believe this to be significantly affecting the results.

None of the previously proposed methods learned anything on the formation control task, in the partial observability/restricted communication setting, or with $M \ge 6$ agents, hence we do not report those results in the table.

\begin{table}[h]
\caption{Comparisons with previous work on coverage control with $M=3$ and $M=6$ agents. \texttt{Av.Dist.} refers to the average distance of a landmark to its closest agent (lower is better). }
\label{tab:prevwork}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccccc}
\toprule
& Observ- & & \multicolumn{2}{c}{$M=3$} & \multicolumn{2}{c}{$M=6$}  \\
Method & ability & Comms & Av. Dist. & S$\%$ & Av. Dist. & S$\%$\\
\midrule
MADDPG\footnotemark{} & Full & N/A & 0.59 & 0 & 0.56 & 0\\
Q-Mix & Full & N/A & 0.19 & 20 & 2.87 & 0\\
VDN & Full & N/A & 0.41 & 0 & 0.46 & 0\\
IQL & Full & N/A & 0.351 & 0 & 0.529 & 0\\
\midrule
Ours: MHA & Partial & RC & \textbf{0.067} & \textbf{91} & 0.103 & 55 \\ % 202,197
Ours: Exp & Partial & RC & 0.074 & 85 & \textbf{0.078} & \textbf{73}\\ % 194, 193
Ours: Uniform & Partial & RC & 0.082 & 84 & 0.11 & 53 \\ % 195, 196
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

% \begin{table}[h]
% \caption{Comparisons with previous work on coverage control with $M=3$ and $M=6$ agents. \texttt{Av.Dist.} refers to the average distance of a landmark to its closest agent (lower is better). }
% \label{tab:prevwork}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lcccccc}
% \toprule
% & Observ- & & \multicolumn{2}{c}{$M=3$} & \multicolumn{2}{c}{$M=6$}  \\
% Method & ability & Comms & Av. Dist. & Success $\%$ & Av. Dist. & Success $\%$\\
% \midrule
% MADDPG & Full & N/A & 0.59 & 0 & 0.56 & 0\\
% Q-Mix & Full & N/A & 0.19 & 20 & 2.87 & 0\\
% VDN & Full & N/A & 0.41 & 0 & 0.46 & 0\\
% IQL & Full & N/A & 0.351 & 0 & 0.529 & 0\\
% Ours & Partial & RC & 0.067 & 91 & 0.103 & 55 \\ % 202,197
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}
% \footnotetext{The official implementation of MADDPG \url{https://github.com/openai/maddpg} could not reproduce the results reported in the paper, hence they have been directly reported (without being verified by us)}

\subsection{Flexibility in message passing}
\label{sec:messagepassingcompare}
Having established that our proposed method with the shared agent-entity graph and learned communication clearly outperforms previously proposed MARL algorithms, we now compare variations of the proposed method. Table \ref{tab:mpcomparison} presents the performance of the 3 different inter-agent message passing functions in both the restricted and unrestricted communication scenarios, as well as the coverage and formation control tasks. It is clear that all 3 functions perform very well, with no function being clearly the best (or worst) in all scenarios. 

Using multi-head attention (MHA) for message passing outperforms exponential kernel and uniform attention, since it gives agents greater selectivity in choosing which neighbors' messages to attend to. We note that MHA has a greater advantage in the unrestricted communication settings, where agents are receiving a large number of messages (from all other agents, rather than only from those within a neighborhood) and hence find the ability to listen selectively more useful, as compared to the restricted communication setting, where agents receive fewer messages, hence ameliorating the effectiveness of MHA.

\begin{table}[h]
\caption{Comparing (1) Multi-Head Attention (MHA), (2) Exponential Kernel Attention (Exp) and (3) Uniform Attention (Uniform) for inter-agent communications on coverage and formation control task, with both unrestricted (UC) and restricted (RC) communication, for $M=\{3,5,6,10\}$ agents.}
\label{tab:mpcomparison}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{ccccccccc}
\toprule
Task & $M$ & Comms & \multicolumn{2}{c}{MHA} & \multicolumn{2}{c}{Exp} & \multicolumn{2}{c}{Uniform} \\
& & & S$\%$ & Time & S$\%$ & Time & S$\%$ & Time \\
\midrule
Coverage & 3 & UC & 96 & 24.14 & 83 & 29.94 & 89 & 26.14\\ % 123,199,200
Coverage & 5 & UC & 100 & 18.41 & 96 & 23.90 & 75 & 33.01\\ % 128,199,200
Coverage & 6 & UC & \textbf{99} & \textbf{20.03} & 87 & 26.15 & 53 & 41.20\\ % 198,199,200
Coverage & 10 & UC & \textbf{98} & \textbf{19.84} & 80 & 29.90 & 0 & 50\\ % 132,199,200
\midrule
Coverage & 3 & RC & 91 & 27.15 & 85 & 28.44 & 84 & 27.8\\ % 202,194,195
Coverage & 5 & RC & 79 & 33 & 78 & 32.69 & 74 & 33.84\\ % 142,177,178
Coverage & 6 & RC & 55 & 39.77 & \textbf{73} & \textbf{35.98} & 53 & 40.52\\ % 197,193,196
Coverage & 10 & RC & 0 & 50 & 0 & 50 & 0 & 50\\ % 209,210,211
\midrule
\midrule
Formation & 3 & UC & 99 & 14.21 & 94 & 17.98 & 90 & 18.63\\ % 185,191,192
Formation & 5 & UC & 99 & 16.55 & 79 & 26.76 & 76 & 28.56\\ % 185,191,192
Formation & 6 & UC & \textbf{99} & \textbf{19.7} & 79 & 28.86 & 77 & 29.53\\ %185,191,192
Formation & 10 & UC & 0 & 50 & \textbf{61} & \textbf{36.75} & 33 & 43.25\\ %212,191,192
\midrule
Formation & 3 & RC & 89 & 20.74 & 96 & 17.38 & 96 & 16.49\\ % 186,204,203
Formation & 5 & RC & 98 & 17.78 & 0 & 50 & 90 & 21.35\\ % 186,204,203
Formation & 6 & RC & \textbf{97} & \textbf{20.52} & 0 & 50 & 66 & 35.55\\ % 186,204,203
Formation & 10 & RC & 8 & 47.69 & 0 & 50 & \textbf{61} & \textbf{35.13}\\ % 186,204,203
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}


% \begin{table}[h]
% \caption{Results of the proposed approach on coverage and formation control task, with both unrestricted (UC) and restricted (RC) communication, for $M=\{3,5,6,10\}$ agents.}
% \label{tab:mpcomparison}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{ccccc}
% \toprule
% Task & $M$ & Comms & Success $\%$ & Time\\
% \midrule
% Coverage & 3 & UC & 96 & 24.14\\ % 123,199,200
% Coverage & 5 & UC & 100 & 18.41\\ % 128,199,200
% Coverage & 6 & UC & 99 & 20.03\\ % 198,199,200
% Coverage & 10 & UC & 98 & 19.84\\ % 132,199,200
% \midrule
% Coverage & 3 & RC & 91 & 27.15\\ % 202,194,195
% Coverage & 5 & RC & 79 & 33\\ % 142,177,178
% Coverage & 6 & RC & 55 & 39.77\\ % 197,193,196
% Coverage & 10 & RC & 0 & 50\\ % 209,210,211
% \midrule
% \midrule
% Formation & 3 & UC & 99 & 14.21\\ % 185,191,192
% Formation & 5 & UC & 99 & 16.556\\ % 185,191,192
% Formation & 6 & UC & 99 & 19.7\\ %185,191,192
% Formation & 10 & UC & 0 & 50\\ %212,191,192
% \midrule
% Formation & 3 & RC & 89 & 20.74\\ % 186,204,203
% Formation & 5 & RC & 98 & 17.78\\ % 186,204,203
% Formation & 6 & RC & \textbf{97} & \textbf{20.52}\\ % 186,204,203
% Formation & 10 & RC & 8 & 47.69\\ % 186,204,203
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}

\subsection{Zero-Shot Generalization to Additional Team Members}
\label{sec:zeroshot}
This subsection looks at what happens when agents are removed or added to the team. Table \ref{tab:generalization} presents results of how policies learned using our framework (using \texttt{MHA} for inter-agent communication) generalize to scenarios when up to 2 team members are added or removed. The presented results are with \textbf{no additional fine-tuning} on the new scenario. 

In the coverage task we see the agents adapting very well to the removal or addition of team members, especially in the unrestricted communication case - achieving up to 99\% accuracy after the loss of 2 teammates. In the formation task, while zero-shot transfer success rates are 0\%, this is because our evaluation of success is a very strict condition. The reward values show us that there is significant transfer of learning, and the policies are very quickly able to adapt to the new scenarios (with only a few gradient updates). We emphasize that this generalization is a direct result of our proposed learning framework, not a result of having exposed the agent to such diversity (in the number of agents) during training (which is the usual practice in multi-task learning).

\begin{table*}
\caption{Zero Shot Generalization: What happens when up to two team members are added or removed from the team? \texttt{S$\%$} is success rate, and \texttt{R} is the average reward received by the agents at the final step of each evaluation episode. The policies were trained with $N$ agents, and the 2 columns marked $N-1$ and $N-2$ indicate performance when 1 and 2 agents, respectively, are removed, while columns marked $N+1$, $N+2$ indicate performance when 1 and 2 agents, respectively, are added.}
\label{tab:generalization}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{cccccccccccc}
\toprule
Task & Comms & \multicolumn{2}{c}{$N$-2} & \multicolumn{2}{c}{$N$-1} & \multicolumn{2}{c}{$N$} & \multicolumn{2}{c}{$N$+1} & \multicolumn{2}{c}{$N$+2}\\
& & S$\%$ & R & S$\%$ & R & S$\%$ & R & S$\%$ & R & S$\%$ & R\\
\midrule
Coverage & UC & 99 & -0.57 & 97 & -0.52 & 96 & -0.47 & 78 & -0.36 & 39 & -0.29\\ % using 131/ep1400
Coverage & RC & 43 & -0.839  & 60 & -0.629 & 79 & -0.59 & 29 & -0.46 & 6 & -0.48\\ % using 142/ep12200
\midrule
Formation & UC & 0 & -0.34 & 0 & -0.26 & 100 & -0.43 & 0 & -0.36 & 0 & -0.47\\ % using 185/ep4500
Formation & RC & 0 & -0.33 & 0 & -0.26 & 97 & -0.52 & 0 & -0.36 & 0 & -0.47 \\ % using 186/7/ep1750
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

\subsection{Robustness to Communication Drops}
\label{sec:robust}
We now look at the performance of learned policies under conditions where the communications networks are glitchy. To encourage robustness to such problems, we trained the agents with dropout communication (Section \ref{sec:dropout}). In both coverage and formation control, agents trained with dropout communication remain robust to random packet loss. More interestingly, we also observed an (unexpected) regularization effect, where training with communication dropout actually improved learning to be better than in the case with perfect communication! This can be seen in Table \ref{tab:regularization}, where the success rate of formation control with $M=10$ agents, in both unrestricted and restricted communication settings, goes from low single-digit success rates to near-perfect (100\%) success rates. Both our technique, and this regularization effect, are similar to dropout \cite{srivastava2014dropout} used for reducing overfitting in deep neural networks.

\begin{table}[h]
\caption{Regularization effects of communication dropout}
\label{tab:regularization}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{cccccc}
\toprule
Task & $M$ & Comms & Dropout & Success $\%$ & Time\\
\midrule
Formation & 10 & UC & No & 0 & 50\\ %212
Formation & 10 & UC & Yes & 97 & 22.85\\ % 208
\midrule
\midrule
Formation & 10 & RC & No & 8 & 47.69\\ % 186
Formation & 10 & RC & Yes & 100 & 20.95\\ % 216
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}


% \begin{table*}
% \caption{Zero Shot Generalization}
% \label{tab:generalization}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{cccccccc}
% \toprule
% Task & Comms & Transfer & Transfer & \multicolumn{2}{c}{Zero-Shot} & \multicolumn{2}{c}{Final}\\
% & & From & To & Success & Time & Success & Time\\
% \midrule
% Coverage & UR & 3 & 5 & 87 & 24.33 & 100 & 10.40\\ %128,123
% Coverage & UR & 5 & 7 & 66 & 40.30 & 97 & 19.9\\ %131
% Coverage & UR & 7 & 10 & 20 & 47.20 & 96.67 & 18.9\\ %132
% \midrule
% Coverage & R & 3 & 5 & 43.33 & 39.60 & 84 & 33.67\\ %142
% Coverage & R & 5 & 7 & 19 & 47.8 & 40 & 43.47 \\ %178
% Coverage & R & 7 & 10 & & & & \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table*}


==> thesis_files/methods.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{figs/SharedAgentEntityGraph.png}
    \caption{The proposed shared agent-entity graph on the right, and a detailed look at the internal architecture of each agent on the left. Agents are in green, environmental entities in blue. Messages are exchanged between agents along the red edges, and are sent from entities to agents along the blue edges. Many agent pairs ($<1,3>,<1,4>,<2,4>$) do not communicate directly, however information from one agent is still able to propagate to others due to the use of multihop communication. 
    The agent state encoder is described in Section \ref{sec:agentstateencoder}, communications in Section \ref{sec:comms} and policy/value heads in Section \ref{sec:policyvalueheads}.}
    \label{fig:overall}
\end{figure}

There are $N$ agents interacting and jointly performing a task, sharing a policy parameterized by $\pi$. Agent $i$ encodes its own state (consisting of information like position, velocity etc.) into a $H$-dim vector, and combines it with information about environmental entities (like landmarks, obstacles etc.) to form an agent embedding $H_i$. The agents then communicate with their neighbors to update their embeddings with the received messages. This is the crucial step which allows the emergence of coherent cooperative behavior in the team. Finally, this updated state is fed to an actor-critic network, whose policy network is used by the agent to choose an action for the environment. The agents then act simultaneously on the environment, and receive a reward which is used to train, in an end-to-end fashion, the entire network architecture, using reinforcement learning. In this work, we consider scenarios where all the agents form a homogeneous team and share policy and value network parameters. Since each agent receives different observations (their own state), sharing parameters does not preclude them from behaving differently, as is appropriate. 
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figs/proposed_framework.png}
    \caption{Agents and entities embedded in a shared graph, with the agents acting upon and receiving a reward from the environment. This figure should be compared to those in Section \ref{sec:prevwork}.}
    \label{fig:framework}
\end{figure}

Figure \ref{fig:overall} provides a high-level overview of the proposed multi-agent learning framework, with the shared agent-entity graph on the right and the internal architecture of each agent on the left. We now describe each part in detail.

\section{Agent-Entity Graph}
\label{sec:graph}
The salient parts of our environment can often be described as a collection of different entities. For a vehicle, this might include traffic lights, pedestrians or obstacles on the road. Any cooperative multi-agent system will also have $M$ agents sharing the environment, who collectively need to accomplish a given objective. We would like each agent to be able to learn to focus selectively on particular entities salient to it (such as obstacles close to it, or objects which align with its goal). Hence, we let the agents receive messages from each entity, where the agent can use attention to selectively focus on all the messages it is receiving.

Hence, we define a graph $G := (V,E)$ where each node $n \in V$ is an agent or an environment entity, and there exists an edge $e \in E$ between two nodes if the agents or entities on those nodes communicate with each other. This can be seen in Figure \ref{fig:overall}.
A shared agent-entity graph has these agents and entities occupying vertices of the graph, with edges existing between those vertices whose occupants can communicate with each other. In a real world scenario, communication is often restricted to within a certain radial distance only, as illustrated in Fig. \ref{fig:restrictedcomms}. 
In the case there is no restriction on communication radius, this graph is fully connected, whereas in the case that communication is restricted to neighbors (agents within the communication radius of each agent), the graph can have arbitrary connectivity, including multiple disconnected components. 
Modeling the agent network as a graph provides a very strong inductive bias to the learning algorithm. In practice, agents which are closer to each other have a greater impact on each others' behavior, and this crucial information is baked into the architecture of the graph, which greatly aids learning. 
Using appropriate message-passing functions in the graph (as discussed below) also enables the learned policies to work in environments with a different number of agents, which is necessary for enabling the agents to learn robust and generalizable strategies.
We now discuss what messages are sent and received between vertices on this graph, and how they use that information to make a decision.

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figs/restricted_comms.png}
    \caption{Illustration of restricted communication. The circles around each agent indicate its radius of communication $R$. Note that the yellow agent is disconnected from the rest of the graph, creating multiple disconnected components which can not communicate with one another. This is a situation encountered frequently in reality and the learned behavior needs to be robust to such situations.}
    \label{fig:restrictedcomms}
\end{figure}

\section{Learning Communication}
\label{sec:comms}
\begin{figure}
    \centering
    \includegraphics[width=0.6\textwidth]{figs/attention.png}
    \caption{Illustration of communication between agents and/or entities, using dot-product attention and multihop routing.}
    \label{fig:attention}
\end{figure}

Communication between agents is crucial for emergence of cooperative behavior. While there has been prior work \cite{agarwal2018community} on goal-oriented communication between two agents grounded in natural language, our focus here is to allow groups of agents to develop a communication protocol, and we do not impose the constraint of natural language grounding.

\subsubsection{Calculating a message to send} All nodes $n$ in the graph (agents and entities) compute a message $v_n^t$ to send, conditioned on their state $h_n^t$:
\[
v_n^t = W_V h_n^t \in \mathbb{R}^{D_V}
\]
where $W_V \in \mathbb{R}^{D_V \times H}$ is a learnable matrix.

\subsubsection{Aggregating received messages} Only agents receive messages. Agent $m$ receives multiple messages from its neighbors in the graph and aggregates them using a weighted linear combination:
\[
M_m^t = \sum_{n}\left(\frac{\exp{(w_{mn}^t)}}{\sum_{n}\exp{(w_{mn}^t)}}\right) v_n^t
\]
where $n$ indexes over all agents (including $m$), and the \texttt{softmax} normalization of the weights $w_{mn}^t$ is done to ensure invariance to the number of agents.
We now discuss how these weights are calculated.

\subsubsection{Calculation of attention weights $w_{mn}^t$}
We use the dot-product multi-head attention mechanism proposed by \citet{vaswani2017attention} to calculate the weight (or attention) that each agent assigns to each message received by it. This weight is a function of the internal state of the agent sending the message and the agent receiving the message. This provides us with two benefits: (1) allows each agent to learn to selectively attend to entities that are more relevant to it,  and (2) ensures invariance and robustness to number of entities in the environment, since the \texttt{softmax} operation in the attention calculation normalizes over the number of agents or entities. 

More specifically, for each vertex in the graph, we calculate a key-value pair $<k_n^t,v_n^t>$ where
\begin{gather*}
k_n^t = W_K^{AE} e_n^t \in \mathbb{R}^{D_K} \\
v_n^t = W_V^{AE} e_n^t \in \mathbb{R}^{D_V}
\end{gather*}
where $W_K^{AE} \in \mathbb{R}^{D_K \times H}$ and $W_V^{AE} \in \mathbb{R}^{D_V \times H}$. 
Each agent vertex $m$ also calculates a query vector $q_m^t = W_Q^{AE} a_m^t \in \mathbb{R}^{D_K}$, where $W_Q^{AE} \in \mathbb{R}^{D_K \times H}$ and $a_m^t$ is the state of the vertex at time $t$. Intuitively, $W_K^{AE}$ and $W_Q^{AE}$ are learnable matrices which embed the states of the two agents (or entity-agent pair) sending and receiving the message, respectively, into a shared embedding space where we can use the dot-product between the two embeddings (key and query, respectively) to compute their similarity. $W_V^{AE}$ is also a learnable matrix which computes a message (value) to be sent from vertex $n$ to the vertices it is connected to (able to communicate with).
\[
        w_{mn}^t = \begin{cases} 
        \left(\dfrac{q_m^t k_n^{t\mathsf{T}}}{\sqrt{D_K}}\right) & \text{if m and n are connected} \\
        -\infty & \text{otherwise}
        \end{cases} \\
\]
where the scaling factor $\frac{1}{\sqrt{D_K}}$ is added for stability \cite{vaswani2017attention} and $j$ indexes over all the agents or entities in the environment. This computation is also depicted in Figure \ref{fig:attention}.

We note that our shared agent-entity graph is also compatible with two previously proposed functions for inter-agent communication, which we specify below for completeness:\\
% This agent-environment encoding $h_i^t$ incorporates information from environmental entities as well as the agent's own state, and is now used for communicating with other agents. Going forward, we refer to $h_i^t$ as the agent's state.
\textbf{Exponential Kernel Attention (VAIN \cite{hoshen2017vain}): }
Each agent computes a key value $k_n^t \in \mathbb{R}^1$:
\[
k_n^t = W_K h_n^t \in \mathbb{R}^1
\]
We then calculate the $L_2$ distance between the key values of agents $m$ and $n$ to use as the attention weight $w_{mn}^t$:
\[
w_{mn}^t = \begin{cases} 
    - || k_m - k_n ||^2 & \text{if m and n are connected} \\
    -\infty & \text{otherwise}
    \end{cases} \\
\]
\textbf{Uniform Attention (CommNet \cite{sukhbaatar2016learning}): }
The agent focuses uniformly on all the messages it receives, i.e.
\[
w_{mn}^t = \begin{cases} 
    1 & \text{if m and n are connected} \\
    -\infty & \text{otherwise}
    \end{cases} \\
\]

\subsubsection{Agent State Update}
The aggregated message $M_m^t$ is now passed through the agent update function $g$, which takes as input the concatenation of the current agent state $h_m^t$ and the aggregated message, to update the agent state.
\[
h_m^t \gets g(h_m^t | M_m^t)
\] where $|$ denotes concatenation.
We emphasize that the matrices $W_K,W_Q,W_V$ and function $g$ are shared (have the same value) across all agents.

\subsubsection{Multi-Hop Communication}
Since the agent graph is sparsely connected, we use multihop (or peer-to-peer) communication to allow information to propagate between agents that might not be directly connected with each other. At each timestep $t$, the message passing algorithm outlined above is repeated $C$ times, after which the hidden state of each agent (potentially) incorporates information from agents up to $C$ hops away. The premise of multi-hop communication is explained in Figure \ref{fig:multihop}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figs/multihopcomm.png}
    \caption{An illustration of information propagation through multi-hop communication. In the first step, the central node has some information (green) which it has to propagate to the other nodes in the graph. In this step, the edges connected directly to the green node carry this information. In the second step, we see that the nodes directly connected to the central node have received this information (have turned green), and now all the edges connected to any green node carry this information. In the third step, we see that nodes which are \textbf{not directly connected} to the central node have also received the information (turned green). This is the basic premise of multi-hop communication, where information can pass between nodes that are not directly connected to each other.}
    \label{fig:multihop}
\end{figure}

\section{Internal Agent Architecture}
\subsection{Agent State Encoder}
\label{sec:agentstateencoder}
At each timestep $t$, agent $i$ observes its local state $x_i^t \in \mathbb{R}^{D_I}$, which consists of information like its own position and velocity, and provides it as input to the agent state encoder $q: \mathbb{R}^{D_I} \rightarrow \mathbb{R}^H$, to produce an embedding $a_i^t \in \mathbb{R}^H$.
\[
a_i^t = q(x_i^t)
\]

\subsection{Policy and Value Output Heads}
\label{sec:policyvalueheads}
As discussed in Section \ref{sec:pg}, actor-critic reinforcement learning algorithms require the agent to produce (1) a probability distribution over actions, and (2) a value estimate of the current state. Hence, each agent is equipped with a policy network and a value network. These networks both take as input the agent state $h_i^t$ obtained after $C$ rounds of communication with the other agents. This input contains information about other agents' expected behavior which is crucial for correct estimation of value and producing a policy distribution which leads to a high probability of coherent and cooperative behavior. While each agent's policy and value network can be independent in a scenario where each agent is unique and heterogeneous, a more likely scenario is that agents have specific roles, for e.g., medic, firefighter and police (in a fire response scenario), and all the agents in a particular role share policy and value networks, since they would be expected to behave interchangeably, which desirable behavior results directly from sharing parameters. 
In this document, we consider only scenarios where all the agents involved are homogeneous, and hence share policy and value network parameters. Since each agent receives different observations (their own state), sharing parameters does not preclude them from behaving differently, as is appropriate. 

\section{Training}
\label{sec:training}

\subsection{Multi-Agent PPO}
\label{sec:mappo}
We adapt the Proximal Policy Optimization (PPO) \cite{schulman2017proximal} actor-critic algorithm for multiple agents. During training, we collect the following data from all agents at each timestep:
\begin{enumerate}
    \item Local state and environment observation
    \item Action taken
    \item Log probability value of the policy head for the action chosen
    \item Reward received from the environment
    \item The agent's value estimate for that state
    \item Did the episode end? (True/False)
\end{enumerate}
The reward and value estimates are later used to calculate returns and advantage estimates for each agent, using Generalized Advantage Estimation \cite{schulman2015high}, as described in Section \ref{sec:pg}. Then, we sample a mini-batch of the collected data for the same time steps for all agents, and use that to do a gradient update. Since PPO updates are stable, we are able to use the same experience for multiple updates, improving sample efficiency.

\subsection{Dropout Communication}
\label{sec:dropout}
Real world communication networks are prone to glitches, with lost or corrupted information packets being a regular occurrence. Usually, these dropped connections are not just momentary but do persist for a short duration of time. 

To operate robustly in the real world, agents have to learn to not be too dependent on continuous communication with their neighbors. We induce this behavior by exposing them to artificially severed communications during training. A fraction $p$ of edges in the agent graph are dropped at each timestep, with the particular edges to be dropped being randomly sampled every $K$ timesteps. This technique also draws inspiration from the dropout technique \cite{srivastava2014dropout} used to reduce overfitting and co-adaptation between neurons in deep neural networks, since our objective is also to reduce co-dependence between agents in the agent graph.

\subsection{Curriculum Training}
\label{sec:curriculum}
We make use of curriculum learning \cite{bengio2009curriculum} to train policies in progressively tougher environments as the number of agents increases. Our graph network framework which is adaptable to varying number of agents and landmarks allows us to transfer learned behavior, and shows both strong zero-shot generalization as well as ability to quickly improve in new scenarios with very few gradient updates.
We deploy a curriculum over the number of agents, i.e. a policy is trained with $M=3$ agents, then transferred (and further trained) with $M=5$ agents, and so on. 

This allows us to vastly simplify the multi-agent credit assignment problem which arises with a large number of agents in cooperative teams, where it is not clear which agent's behavior might be leading to a reward or penalty from the environment. In the $3$ agent case, the credit assignment problem is not very difficult - and then the use of a curriculum when scaling to larger teams makes sure that the agents always have a very strong policy to bootstrap from.

==> thesis_files/preliminaries.tex <==
In this chapter we introduce preliminary concepts required to understand this thesis, and expose related prior work to put our work in context.

\section{Reinforcement Learning}
\label{sec:rl}
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figs/background_rl.png}
    \caption{The classic reinforcement learning "Observation - Action - Reward" loop. An agent observes its environment and uses this information to act appropriately upon the environment, which in turn transitions to a new state and rewards or penalizes the agent based on the objective at hand. The agent learns to choose its actions such that the long-term discounted reward it receives is maximized.}
    \label{fig:background_rl}
\end{figure}

\subsection{Markov Decision Processes}
\label{sec:mdp}
In the real world, an agent's actions influence not just the immediate rewards it receives, but also the subsequent state of the environment, which in turn influences future rewards. This kind of sequential decision-making process is often formalized as a Markov Decision Process (MDP). An MDP is defined by a tuple $(S,A,P,r,p_0,\gamma)$ where $S$ is a finite set of states, $A$ is a finite set of actions, $P: S \times A \times S \rightarrow \mathbb{R}$ is the state transition probability distribution, $r: S \rightarrow \mathbb{R}$ is the reward function, $p_0: S \rightarrow \mathbb{R}$ is the probability distribution over the agent's initial state $s_0$, and $\gamma$ is the discount factor which determines how much the agent values immediate rewards over future rewards. 
The name derives from the Markov property, which describes processes whose future state depends only on the present state, not on the sequence of events that preceded it. This can be formalized as $p(s_{t+1}|s_{t},a_{t},\cdots,s_0,a_0) = p(s_{t+1}|s_t,a_t)$

The policy is a probability distribution from states to actions $\pi : S \times A \rightarrow [0,1]$ which encodes the agent's probability of taking each action in each state. 
Under policy $\pi$, the state value function $V_{\pi} : S \rightarrow \mathbb{R}$, action-value function $Q_{\pi} : S \times A \rightarrow \mathbb{R}$ and advantage function $A_{\pi}(s_t,a_t)$ are defined as:
\begin{gather*}
    Q_{\pi}(s_t,a_t) = \mathbb{E}_{s_{t+1},a_{t+1},\cdots} \sum_{k=0}^{\infty} \gamma^k r(s_{t+k}) \\
    V_{\pi}(s_t) = \mathbb{E}_{a_t,s_{t+1},a_{t+1},\cdots} \sum_{k=0}^{\infty} \gamma^k r(s_{t+k}) \\
    A_{\pi}(s_t,a_t) = Q_{\pi}(s_t,a_t) - V_{\pi}(s_t)
\end{gather*}
where $a_t \sim \pi(a|s_t), s_{t+1} \sim p(s_{t+1}|s_t,a_t)$, and the subscripts $t,t+1$ etc. refer to time. 

\subsection{Policy Gradient methods for learning in MDPs}
\label{sec:pg}
An agent's objective is to maximize the expected total discounted reward $\sum_{k=0}^{\infty} \gamma^k r(s_{t+k})$.
Let the policy $\pi$ be parameterized by $\theta$. Policy gradient methods \cite{williams1992simple} usually optimize this by estimating the gradient $g = \nabla_{\theta} \mathbb{E} \sum_{k=0}^{\infty} \gamma^k r(s_{t+k})$.
This has multiple formulations which tradeoff bias and variance in the resulting gradient estimate, however for the purpose of this thesis we will use the following:
\[
\hat{g} = \mathbb{\hat{E}} \sum_{t=0}^{\infty} \hat{A}_{\pi,\gamma}(s_t,a_t) \nabla_{\theta} \log \pi_{\theta} (a_t|s_t)
\]
where $\hat{A}$ is an estimate of the advantage function, using the Generalized Advantage Estimator (GAE) \cite{schulman2015high}, and $\mathbb{\hat{E}}$ denotes the empirical average over a finite batch of samples.
\begin{gather}
\label{eq:gae}
    \hat{A}_t^{GAE(\gamma,\lambda)} = \sum_{l=0}^{\infty} (\gamma\lambda)^l \delta_{t+l}^V \\
    \delta_t^V = r_t + \gamma V(s_{t+1}) - V(s_t)
\end{gather}
where $\gamma$ is the discount factor, and $\lambda$ is a hyperparameter which contributes to the bias-variance tradeoff. Note that the agent needs to maintain an estimate of the value function $V$, along with its estimate of the policy $\pi$, in order to use this formulation of the policy gradient method.

To improve stability and robustness to hyperparameter settings, we use the PPO algorithm \cite{schulman2017proximal} which optimizes a clipped, surrogate policy gradient objective function. This algorithm has subsequently been used in many works \cite{agarwal2018challenges,OpenAI_dota} for its stability and robustness to hyperparameter settings.

\begin{gather}
\label{eq:lclip}
L^{CLIP}(\theta)=\hat{\mathbb{E}}_{t}\left[\min \left(r_{t}(\theta) \hat{A}_{t}, \operatorname{clip}\left(r_{t}(\theta), 1-\epsilon, 1+\epsilon\right) \hat{A}_{t}\right)\right] \\
r_{t}(\theta)=\frac{\pi_{\theta}\left(a_{t} | s_{t}\right)}{\pi_{\theta_{\text {old}}}\left(a_{t}|s_{t}\right)}
\end{gather}where $\theta_{\text{old}}$ is the vector of policy parameters before the update. The second term inside the $\min$ removes the incentive for moving $r_t$ outside of the interval $[1-\epsilon,1+\epsilon]$, preventing potentially harmful major updates to the policy and lending to stability of training. We also add a MSE (L-2) loss function for the value estimate, and add an entropy bonus to encourage exploration. This leads to the final objective function for PPO:
\begin{equation}
\label{eq:ppo}
    L:= L_{t}^{C L I P+V F+S}(\theta)=\hat{\mathbb{E}}_{t}\left[L_{t}^{C L I P}(\theta)-c_{1} L_{t}^{V F}(\theta)+c_{2} S\left[\pi_{\theta}\right]\left(s_{t}\right)\right]
\end{equation}
 where $c_1,c_2$ are coefficients, $S$ denotes the entropy bonus, and $L_{t}^{V F}$ is a squared error loss $\left(V_{\theta}\left(s_{t}\right)-V_{t}^{\operatorname{targ}}\right)^{2}$. For completeness, we present the PPO algorithm from \citet{schulman2017proximal}.

\begin{algorithm*}
\caption{Proximal Policy Optimization (PPO)}
\label{alg:ppo}
\begin{algorithmic}[1]
\State Initialize $\pi_{\theta}, V_{\theta}$
\For{$\text{iter}=1,2,\cdots$}
\State Run policy $\pi_{\theta_{\text{old}}}$ in $N$ parallel environments for $T$ timesteps.
\State Compute GAE advantage estimates $\hat{A}$ for each timestep in each environment.
\For{$\text{k}=1,\cdots,K$}
\State Construct $L$ using Eqn. \ref{eq:ppo} and optimize wrt $\theta$, with minibatch size $M \leq NT$.
\State $\theta_{\text{old}} \gets \theta$
\EndFor
\EndFor
\end{algorithmic}
\end{algorithm*}

\subsection{Markov Games} 
The standard single-agent RL setting assumes that a single agent acts on the environment, and has to, by definition, treat other agents as part of the environment. Instead, we model multi-agent environments as Markov (or stochastic) games, which are a generalization of MDPs to the multi-agent setting first proposed by \citet{littman1994markov}. We note that in the fully cooperative case, this formulation is consistent with the decentralized partially observable MDPs (Dec-POMDP) formulation \citet{oliehoek2016concise}.

Defined by a tuple $(S,\textbf{A},P,r,\gamma,N,\textbf{Z},O)$ where $N$ is the number of agents, $S$ is the set of states, $P: S \times \textbf{A} \times S \rightarrow [0,1]$ is the state transition probability function. At each time step, each agent chooses an action $a^i \in \textbf{A}$, to create a joint action $\textbf{a} \in \textbf{A}^n$, and receives an immediate reward from the environment $r^i(s,\textbf{a}): S \times \textbf{A} \rightarrow \mathbb{R}$, along with an observation $z^i \in Z$ according to observation function $O(s,a): S \times A \rightarrow Z$. Each agent's policy $\pi^i$ is conditioned on its history of observations and actions, $h^i \in H \in (Z \times A) $.
We consider fully cooperative games, where all agents share the same reward function and discount factor. 

\section{Related Work in Multi-Agent RL}
\label{sec:prevwork}

Following the success of deep RL in single-agent domains \cite{silver2016mastering,mnih2015human}, there has been a resurgence in multi-agent RL led by the use of deep neural networks to parameterize agent policies or value functions, allowing methods to tackle high-dimensional state and action spaces. Having looked at single-agent RL in the previous section, we now discuss various formulations of the multi-agent reinforcement learning problem.

\subsection{Centralized Multi-Agent RL}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.35\textwidth]{figs/background_marl_hivemind.png}
    \caption{Multi-Agent Reinforcement Learning with a Hive Mind (centralized controller)}
    \label{fig:background_marl_hivemind}
\end{figure}
Centralized multi-agent RL (see Figure \ref{fig:background_marl_hivemind}) is the simplest, most obvious interpretation of multi-agent RL. There is a centralized controller, or a “hive mind”, which receives information from all the agents in the system, and then takes a collective decision about what action each agent should take. Being able to consider a wide variety of information from all the agents and then order each agent around makes this very powerful. It can be thought of as a single-agent system with multiple arms that it can directly control, the same way we have full control over our own two arms. Hence, from a learning perspective, this is effectively single-agent reinforcement learning. 
The recent paper on AlphaStar by DeepMind \cite{alphastarblog} which has demonstrated superhuman performance on the challenging multi-agent game of StarCraft treats the problem in such a fully centralized manner. It is worthwhile to note that such a centralized approach is hard to scale to many agents, since the observation and action spaces grow combinatorially, leading to an explosion of the policy search space, meaning that converging to a good policy becomes very difficult, and computationally expensive, often out of reach for academic research labs.
Another disadvantage of such a system is that it has a single point of failure. Any event impacting the central controller's ability to command the agents renders all the agents useless. This fragility is obviously undesirable.

\subsection{Decentralized Multi-Agent RL}
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.6\textwidth]{figs/background_marl_decentralized.png}
    \caption{Fully decentralized multi-agent reinforcement learning - each agent is an independent decision making entity, relying solely on its own observation $O_i$ to choose an action $A_i$.}
    \label{fig:background_marl_decentralized}
\end{figure}
To mitigate these drawbacks, we consider a decentralized setting now, where each agent is its own decision making entity, which receives its own observation from the environment and chooses to act solely on this observation. 
The observation received by each agent usually consists of information within a certain observability radius of the agent. If there are other agents within that radius, they can observe each other. 
The benefits of this approach include the absence of a single point of failure, which means that even if anything happens to one agent - the rest can carry on. Decentralization also makes scaling (up to larger teams) easier, since each agent is only observing its local area.

There has been a lot of work in this problem setting, which we now discuss.
Independent Q-learning \cite{tan1993multi,tampuu2017multiagent} requires training independent Q-value functions for each agent using regular Q-learning \cite{watkins1992q}, while assuming that the other agents are a part of the environment. Since the other agents are also learning, the environment becomes non-stationary and the resulting instability has prevented these methods from working with more than 2 agents in simple settings. 
Other works like \cite{omidshafiei2017deep,matignon2007hysteretic} present a formalization of multi-agent decentralized RL under partial observability and also address learning stabilisation, and present results on normal form games or predator-prey games with up to 3 agents. However, these methods do not scale to a larger number of agents.
Under the paradigm of centralised learning with decentralised execution, a multitude of recent works have trained actor-critic algorithms where the critic is centralized and makes use of global information during training, allowing the agents to use only the actor network to execute in a fully decentralized manner. 
MADDPG \cite{lowe2017multi} learns a centralised critic for each agent by providing the actions of all agents to the critics, and train different policies for each agent using the DDPG algorithm. They present results in cooperative and competitive environments with up to 3 agents, and we compare our results with this algorithm in Section \ref{sec:experiments}. 
COMA \cite{foerster2018counterfactual} also uses a centralised critic but estimates a counterfactual advantage function that helps with multi-agent credit assignment by isolating the effect of each agent's action. They present results with up to 5 agents in Starcraft unit micromanagement tasks. These fully centralized critics becomes impractical as we increase the number of agents. 
VDN \cite{sunehag2017value} counter this by decomposing a centralized state-action value function into a sum of individual agent specific functions and present results on 2-agent grid world environments. The decomposition introduced imposes a strict prior which is not well justified, and limits the complexity of the agents' learned value functions. 
Q-Mix \cite{rashid2018qmix} improves upon this by removing the requirement of additive decomposition of the centralised critic, instead imposing a less restrictive monotonicity requirement on agents' individual state-action value functions, and allowing a learnable mixing of the individual functions which does not limit the complexity of functions that could be learned. This paper also presents results with up to 8 agents in a variety of StarCraft unit micromanagement tasks. 
To the best of our knowledge, all these works using a centralized critic use network architectures which prevent any transfer of learned behavior to environments with greater or fewer number of team members. These papers do not study robustness of learned behavior to addition or deletion of team members, or, more broadly, generalization via extrapolation to any domain not seen during training. 

A significant drawback of this approach is that the agents can’t actually coordinate with each other during execution - they depend myopically on their own observations. If the agents encounter a situation never before seen during training, there is no mechanism which allows them to adapt to that.

\subsection{Decentralized Multi-Agent RL with Communication}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\textwidth]{figs/background_marl_decentralized_with_comms.png}
    \caption{Decentralized multi-agent reinforcement learning, where the agents are allowed to communicate with each other. Agent $i$ receives observation $O_i$, communicates with other agents and gathers information $M$, and then chooses an action $A_i$.}
    \label{fig:background_marl_comms}
\end{figure}
To ameliorate this significant weakness, we can allow the agents to start communicating with each other, along the red arrows between the agents. This communication is usually learned, and could consist of symbols from a discrete vocabulary or, of vectors of real numbers. While the agents still observe local information, they are able to communicate with each other during execution, which provides a mechanism for them to adapt to scenarios never seen before during training. This communication is often restricted, either due to bandwidth considerations, or to be within a certain radial distance only.

CommNet \cite{sukhbaatar2016learning} is one of the earliest works to learn a differentiable communication protocol between multiple agents in a fully cooperative setting, and presented results on interesting cooperative tasks like a traffic junction, however they work with a fully centralized communication architecture and full observability. The paper does not explicitly model interactions between agents, instead each agent receives the averaged states of all its neighbors. 
VAIN \cite{hoshen2017vain} remedied this by using an exponential kernel based attention to weigh the other agents' states, and effectively demonstrated predictive modeling of multi-agent systems using supervised learning. 
\citet{mordatch2018emergence} also demonstrated emergence of compositional language in multi-agent systems with up to 3 agents in both cooperative and competitive settings, and released a multi-agent particle environment which we make use of in this work. They, however, learned discrete communication using symbols from a limited vocabulary, and made it end-to-end differentiable by using the Gumbel-softmax estimator in a fully centralized approach. 
ATOC \cite{jiang2018learning} proposes an attentional communication model that learns when communication is needed and dynamically creates cliques which can communicate among each other using a bidirectional LSTM unit as the channel.

In work done concurrently to ours, TarMAC \cite{das2018tarmac} uses a scaled dot-product attention mechanism for inter-agent communication, and present results in a 3D indoor navigation task. They do not impose any restrictions on communication, leading to a centralized execution paradigm. DGN \cite{jiang2018graph} also uses a similar mechanism for inter-agent communication, using Q-learning for training. They restrict each agent to communicate with its 3 closest neighbors. From a practical consideration, communication between agents is usually restricted by distance, meaning that an agent can communicate only with neighbors within a certain radius. For example, this is the standard practice in the swarm robotics community. We would also like to emphasize that being able to communicate with the 3 closest neighbors ensures that the agents' graph is always a single connected component and no agent is ever disconnected from the others, while having a distance-based restriction leads to formation of several different connected components in the agents' graph, none of which can communicate with each other - leading to a significantly more difficult learning (to cooperate) problem. 
